SurfaceNet: An End-to-end 3D Neural Network for Multiview Stereopsis

This paper proposes an end-to-end learning framework for multiview stereopsis. We term the network SurfaceNet. It takes a set of images and their corresponding camera parameters as input and directly infers the 3D model. The key advantage of the framework is that both photo-consistency as well geometric relations of the surface structure can be directly learned for the purpose of multiview stereopsis in an end-to-end fashion. SurfaceNet is a fully 3D convolutional network which is achieved by encoding the camera parameters together with the images in a 3D voxel representation. We evaluate SurfaceNet on the large-scale DTU benchmark.

==> sections/copy.tex <==

\section{Final copy}

You must include your signed IEEE copyright release form when you submit
your finished paper. We MUST have this form before your paper can be
published in the proceedings.

Please direct any questions to the production editor in charge of these
proceedings at the IEEE Computer Society Press: Phone (714) 821-8380, or
Fax (714) 761-1784.



==> sections/discussion.tex <==

%- - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\subsection{discussion and future work}

\textbf{potentials}
1. such 3D network design can be valuable for other 3D applications, such as point cloud denoising and holes filling.
2. the learned 3D kernels could be used to replace the hand-crafted 3D features and descriptors. 
    Consequently, it can be used for the applications like point cloud registration and semantic labeling.
\par

\textbf{future work}
1. speedup using sparse representation of the surface model. (sparseCNN, octreeCNN, ...)
2. combine with semantic information:
    a. combine with the 2D image semantic labels by expanding into the color channels in the colored voxel cube;
    b. directly supervise and infer dense 3D semantic labels.
\par 
% % about the new method's error pattern
% The network learns some surface structure information, which is relatively higher level than voxel level photo consistency method.
% So that it can be more robust to not-too-large pure color regions, for example in the model12 middle part of letters other methods will have small holes.
% 
% problem: repeating pattern and pure color region.
% 
% Interestingly, we haven't use 'pool along the ray' (?) condition yet. 
% The reason we didn't use the postprocessing like hole filling / outlayer rejection is that we want show our new method alone can be competitive to the state of the art methods, some of which have several postprocessing stages.
% 
% 


==> sections/fig/gamma.tex <==

\begin{figure}[htbp]
    \centering
    \newcommand{\colw}{0.45}
    \newcommand{\figw}{1} % can bigger than 1
    \begin{subfigure}[b]{0.8\linewidth}
        \includegraphics[width=1.0\textwidth,trim={0.0cm 0.0cm 0cm 0.0cm},clip]{figures/table/scatter/gamma}
        % \caption{effect of $\gamma$ when $\tau=0.5;0.7$.}
    \end{subfigure}%


    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={8.3cm 6.5cm 15.5cm 7.2cm},clip]{{figures/results/model9/gamma/t0.7_rp0}.jpg}
        \captionsetup{labelformat=empty}
        \caption{$\gamma=0\%$}
    \end{subfigure}%
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={8.3cm 6.5cm 15.5cm 7.2cm},clip]{{figures/results/model9/gamma/t0.7_rp5}.jpg}
        \captionsetup{labelformat=empty}
        \caption{$\gamma=50\%$}
    \end{subfigure}
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={8.3cm 6.5cm 15.5cm 7.2cm},clip]{{figures/results/model9/gamma/t0.7_rp8}.jpg}
        \captionsetup{labelformat=empty}
        \caption{$\gamma=80\%$}
    \end{subfigure}
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={8.3cm 6.5cm 15.5cm 7.2cm},clip]{{figures/results/model9/gamma/t0.7_rp10}.jpg}
        \captionsetup{labelformat=empty}
        \caption{$\gamma=100\%$}
    \end{subfigure}

    \caption{ Quantitative and qualitative evaluation of $\gamma$ for two values of $\tau$. The images are shown for $\tau=0.7$. 
  %  vary the ray pooling parameter $\gamma$ for specific $\tau=0.5;0.7$.
   %     In both cases, the ray pooling operation dramatically improves the accuracy of the reconstruction results.
    %    Not only the ray pooling outputs thinner surface, but some noisy surface can be filtered.
        } 
   \label{fig:gamma}
\end{figure}


==> sections/fig/tau.tex <==

\begin{figure}[htbp]
    \centering
    \newcommand{\colw}{0.30}
    \newcommand{\figw}{1.1} % can bigger than 1
    \begin{subfigure}[b]{0.99\linewidth}
        \includegraphics[width=1.0\textwidth,trim={0.0cm 0.0cm 0.0cm 0.0cm},clip]{figures/table/scatter/tau_gamma}
        % \caption{effect of $\tau$ when $\gamma=0\%; 100\%$.}
    \end{subfigure}%

    % leave a blank line to change row       
    \begin{subfigure}[t]{0.03\linewidth}
        \rotatebox{90}{$\gamma=0\%$}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth]{{figures/results/model9/t0.5_rp0}.jpg}
        % \caption{$\tau=0.5$}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth]{{figures/results/model9/t0.7_rp0}.jpg}
        % \caption{$\tau=0.7$}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth]{{figures/results/model9/t0.9_rp0}.jpg}
        % \caption{$\tau=0.9$}
    \end{subfigure}
    \begin{subfigure}[t]{0.03\linewidth}
        \rotatebox{90}{$\gamma=100\%$}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={8.3cm 6.5cm 15.5cm 7.2cm},clip]{{figures/results/model9/tau/t0.5_rp10}.jpg}
        \captionsetup{labelformat=empty}
        \caption{$\tau=0.5$}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={8.3cm 6.5cm 15.5cm 7.2cm},clip]{{figures/results/model9/tau/t0.7_rp10}.jpg}
        \captionsetup{labelformat=empty}
        \caption{$\tau=0.7$}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{\colw\linewidth}
        \includegraphics[width=\figw\textwidth,trim={8.3cm 6.5cm 15.5cm 7.2cm},clip]{{figures/results/model9/tau/t0.9_rp10}.jpg}
        \captionsetup{labelformat=empty}
        \caption{$\tau=0.9$}
    \end{subfigure}
    \caption{Quantitative and qualitative evaluation of $\tau$ for two values of $\gamma$. 
        %$\tau$ has consistent affection for accuracy and completeness.
        } 
   \label{fig:tau}
\end{figure}


==> sections/formatting.tex <==
\section{Formatting your paper}

All text must be in a two-column format. The total allowable width of the
text area is $6\frac78$ inches (17.5 cm) wide by $8\frac78$ inches (22.54
cm) high. Columns are to be $3\frac14$ inches (8.25 cm) wide, with a
$\frac{5}{16}$ inch (0.8 cm) space between them. The main title (on the
first page) should begin 1.0 inch (2.54 cm) from the top edge of the
page. The second and following pages should begin 1.0 inch (2.54 cm) from
the top edge. On all pages, the bottom margin should be 1-1/8 inches (2.86
cm) from the bottom edge of the page for $8.5 \times 11$-inch paper; for A4
paper, approximately 1-5/8 inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area 6-7/8 inches (17.5 cm) wide by 8-7/8 inches (22.54 cm)
high.



%-------------------------------------------------------------------------
\subsection{Type-style and fonts}

Wherever Times is specified, Times Roman may also be used. If neither is
available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE. Center the title 1-3/8 inches (3.49 cm) from the top edge of
the first page. The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and
adverbs; do not capitalize articles, coordinate conjunctions, or
prepositions (unless the title begins with such a word). Leave two blank
lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type. This information is to
be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT. Type main text in 10-point Times, single-spaced. Do NOT use
double-spacing. All paragraphs should be indented 1 pica (approx. 1/6
inch or 0.422 cm). Make sure your text is fully justified---that is,
flush left and flush right. Please do not place any additional blank
lines between paragraphs.

Figure and table captions should be 9-point Roman type as in
Figures~\ref{fig:onecol} and~\ref{fig:short}.  Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-,
second-, and third-order headings.

FIRST-ORDER HEADINGS. (For example, {\large \bf 1. Introduction})
should be Times 12-point boldface, initially capitalized, flush left,
with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS. (For example, { \bf 1.1. Database elements})
should be Times 11-point boldface, initially capitalized, flush left,
with one blank line before, and one after. If you require a third-order
heading (we discourage it), use 10-point Times, boldface, initially
capitalized, flush left, preceded by one blank line, followed by a period
and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote {This is what a footnote looks like.  It
often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral
observations in
the text (within parentheses, if you prefer, as in this sentence).  If you
wish to use a footnote, place it at the bottom of the column on the page on
which it is referenced. Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times,
single-spaced, at the end of your paper. When referenced in the text,
enclose the citation number in square brackets, for
example~\cite{Authors14}.  Where appropriate, include the name(s) of
editors of referenced books.

\begin{table}
\begin{center}
\begin{tabular}{|l|c|}
\hline
Method & Frobnability \\
\hline\hline
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\hline
\end{tabular}
\end{center}
\caption{Results.   Ours is better.}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.  Please ensure that any point you wish to
make is resolvable in a printed copy of the paper.  Resize fonts in figures
to match the font in the body text, and choose line widths which render
effectively in print.  Many readers (and reviewers), even of an electronic
copy, will choose to print your paper in order to read it.  You cannot
insist that they do otherwise, and therefore must not assume that they can
zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use
\verb+\includegraphics+, and to specify the  figure width as a multiple of
the line width as in the example below
{\small\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.eps}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the CVPR 2017 web page for a discussion
of the use of color in your document.


